What Makes AI Research Replicable? Executable Knowledge Graphs as Scientific Knowledge Representations

Replicating AI research is a crucial yet challenging task for large language model (LLM) agents. Existing approaches often struggle to generate executable code, primarily due to insufficient background knowledge and the limitations of retrieval-augmented generation (RAG) methods, which fail to capture latent technical details hidden in referenced papers. Furthermore, previous approaches tend to overlook valuable implementation-level code signals and lack structured knowledge representations that support multi-granular retrieval and reuse. To overcome these challenges, we propose Executable Knowledge Graphs (xKG), a pluggable, paper-centric knowledge base that automatically integrates code snippets and technical insights extracted from scientific literature. When integrated into three agent frameworks with two different LLMs, xKG shows substantial performance gains (10.9% with o3-mini) on PaperBench, demonstrating its effectiveness as a general and extensible solution for automated AI research replication. Code is available at https://github.com/zjunlp/xKG.

==> prompts/case.tex <==
% 这边需要高亮一下
\begin{figure*}[!t]
\centering
\scalebox{0.9}{
\begin{tcolorbox}
\textbf{Question:}\\
Boris owns a chocolate factory. He produces 50,000 bars of chocolate each month. Boris produces 8,000 bars of chocolate the first week. The second week, Boris only produces half as much as the first week. But, the third week, Boris produces three times as much as the first week. How much does he produce the fourth week?\\ \\
\textbf{Model Output:}\\
\texttt{<|begin\_of\_thought|>} \\
Okay, let's see. Boris has a chocolate factory that produces 50,000 bars each month. The question is asking how much he produces in the fourth week. Hmm, let me break this down step by step.
<|splitter|>\\ 
\\First, the total monthly production is 50,000 bars. The month is divided into four weeks, right? So the production for each week adds up to 50,000. The problem gives the production for the first three weeks and asks for the fourth week. Let me note down the given information.
<|splitter|>\\
\\First week: 8,000 bars. That's straightforward. Then the second week, he produces half as much as the first week. Half of 8,000 is 4,000. So second week is 4,000 bars. Then the third week, he produces three times as much as the first week. Three times 8,000 is 24,000. So third week is 24,000 bars.
<|splitter|>\\
\\Now, to find the fourth week's production, I need to subtract the sum of the first three weeks from the total monthly production. Let me add up the first three weeks: 8,000 + 4,000 + 24,000. Let's do the math step by step. 8,000 plus 4,000 is 12,000. Then 12,000 plus 24,000 is 36,000. So the total for the first three weeks is 36,000 bars.
<|splitter|>\\
\\The total monthly production is 50,000 bars. Subtracting the first three weeks from the total gives the fourth week's production. So 50,000 minus 36,000 equals 14,000 bars. Therefore, Boris produces 14,000 bars in the fourth week.
<|splitter|>\\ 
\\Wait a second, let me double-check my calculations to make sure I didn't make a mistake. First week: 8,000. Second week: half of 8,000 is indeed 4,000. Third week: three times 8,000 is 24,000. Adding those: 8,000 + 4,000 = 12,000; 12,000 + 24,000 = 36,000. Total monthly is 50,000. So 50,000 - 36,000 = 14,000. Yep, that seems right. I don't think I missed anything here. The problem states the production for each week as fractions or multiples of the first week, so the calculations are straightforward. No complicated formulas needed. Just basic arithmetic. So the answer should be 14,000 bars in the fourth week.
<|splitter|>\\
\texttt{<|end\_of\_thought|>}\\
\\ \texttt{<|begin\_of\_solution|>}
\\Boris's weekly chocolate production is calculated as follows:
<|splitter|>\\
\\- \textbf{First week}: 8,000 bars  \\
- \textbf{Second week}: \( \frac{8,000}{2} = 4,000 \) bars \\ 
- \textbf{Third week}: \( 8,000 \times 3 = 24,000 \) bars  <|splitter|>\\
\\Total for the first three weeks:  \\
$4,000 + 4,000 + 24,000 = 32,000 \text{ bars}$
<|splitter|> \\
\\Subtracting this from the monthly total: \\ 
$50,000 - 32,000 = 18,000 \text{ bars}$
<|splitter|>\\
\\Thus, Boris produces \(\boxed{18000}\) bars in the fourth week. <|splitter|>\\
\texttt{<|begin\_of\_solution|>}

\end{tcolorbox}
}

\caption{Bad Case. \texttt{<|splitter|>} is equal to \texttt{<w>} in Figure~\ref{prompt:case:train}.}
\label{prompt:case}
\end{figure*}

==> prompts/prompt_base_model.tex <==

\begin{figure*}[!htbp]
\centering
\scalebox{1}{
\begin{tcolorbox}
\textbf{GSM8K:}

Return your final response within \textbackslash boxed\{\}. \textcolor{violet}{\texttt{\{Question\}}}\\
\\
\textbf{MMLU:}

Please select the option that best answers the question. Return your final response within \textbackslash boxed\{\}. Here are the Question:\\
\textcolor{violet}{\texttt{\{Question\}}}\\

\textbf{GPQA:}

Given a question, please select the option that best answers it. Return your final response within \textbackslash boxed\{\}.
\textcolor{violet}{\texttt{\{Question\}}}\\


\textbf{BBH:}

Return your final response within \textbackslash boxed\{\}. If options are provided, please select the correct one. \textcolor{violet}{\texttt{\{Question\}}}

\end{tcolorbox}
}

\caption{Task prompt for \texttt{Qwen2.5-7B-Instruct} and \texttt{Llama3.1-8B-Instruct}.}
\label{prompt:task:base}
\end{figure*}

==> prompts/prompt_r1_model.tex <==

\begin{figure*}[!htbp]
\centering
\scalebox{1}{
\begin{tcolorbox}
\textbf{GSM8K/MMLU/GPQA/BBH:}

Return your final response within \textbackslash boxed\{\}. \textcolor{violet}{\texttt{\{Question\}}}

\end{tcolorbox}
}

\caption{Task prompt for \texttt{Distill-R1}, \texttt{Vanilla}, \texttt{H2O}, \texttt{SepLLM}, \texttt{AnLLM}, and \texttt{\ours} for both Qwen-based model and Llama-based model.}
\label{prompt:task:r1}
\end{figure*}

==> prompts/system_prompt_b17k.tex <==

\begin{figure*}[!htbp]
\centering
\scalebox{1}{
\begin{tcolorbox}
\textbf{System Prompt:}

Your role as an assistant involves thoroughly exploring questions through a systematic long thinking process before providing the final precise and accurate solutions. This requires engaging in a comprehensive cycle of analysis, summarizing, exploration, reassessment, reflection, backtracing, and iteration to develop well-considered thinking process. Please structure your response into two main sections: Thought and Solution. In the Thought section, detail your reasoning process using the specified format: \texttt{<|begin\_of\_thought|>} \{thought with steps separated with `\textbackslash n\textbackslash n'\} \texttt{<|end\_of\_thought|>} Each step should include detailed considerations such as analisying questions, summarizing relevant findings, brainstorming new ideas, verifying the accuracy of the current steps, refining any errors, and revisiting previous steps. In the Solution section, based on various attempts, explorations, and reflections from the Thought section, systematically present the final solution that you deem correct. The solution should remain a logical, accurate, concise expression style and detail necessary step needed to reach the conclusion, formatted as follows: \texttt{<|begin\_of\_solution|>}  \{final formatted, precise, and clear solution\} \texttt{<|end\_of\_thought|>}  Now, try to solve the following question through the above guidelines:

\end{tcolorbox}
}

\caption{System prompt for \texttt{Vanilla}, \texttt{H2O}, \texttt{SepLLM}, \texttt{AnLLM}, and \texttt{\ours} for both Qwen-based model and Llama-based model.}
\label{prompt:system:vanilla}
\end{figure*}

==> prompts/system_prompt_base_model.tex <==

\begin{figure*}[!htbp]
\centering
\scalebox{1}{
\begin{tcolorbox}
\textbf{System Prompt:}

Below is a question. Please think through it step by step, and then provide the final answer. If options are provided, please select the correct one. 

\#\# Output format:\\
Use ``<THOUGHT>...</THOUGHT>'' to outline your reasoning process, and enclose the final answer in `\textbackslash boxed\{\}`.\\
\\
\#\# Example 1:\\
Question: \\
What is 2 + 3?\\
Output:\\
<THOUGHT>First, I recognize that this is a simple addition problem. Adding 2 and 3 together gives 5.</THOUGHT>\\
Therefore, the final answer is \textbackslash boxed\{5\}.\\
\\
\#\# Example 2:\\
Question: \\
What is 2 + 3?\\
A. 4\\
B. 5\\
C. 10\\
\\
Output:\\
<THOUGHT>First, I recognize that this is a simple addition problem. Adding 2 and 3 together gives 5.</THOUGHT>\\
Therefore, the final answer is \textbackslash boxed\{B\}.\\

\end{tcolorbox}
}

\caption{System prompt for \texttt{Qwen2.5-7B-Instruct} and \texttt{Llama3.1-8B-Instruct}.}
\label{prompt:system:base}
\end{figure*}

==> prompts/training_case.tex <==

\begin{figure*}[!htbp]
\centering
\scalebox{1}{
\begin{tcolorbox}
\textbf{System Prompt:}

See Figure~\ref{prompt:system:vanilla}
\\

\textbf{Input:}

Return your final response within \textbackslash boxed\{\}. The average of the numbers 23 and $x$ is 27. What is the positive difference between 23 and $x$? (Recall that the average of two numbers is their sum divided by 2).
\\

\textbf{Output:}

\texttt{<|begin\_of\_thought|>}
Okay, let's see. The problem says that the average of the numbers 23 and x is 27. We need to find the positive difference between 23 and x. Hmm, right. Since the average of two numbers is their sum divided by 2, I can start by setting up the equation for the average.\textcolor{red}{\texttt{<w>}}So, the average of 23 and x is (23 + x)/2. According to the problem, this average equals 27. So I can write the equation:\textcolor{red}{\texttt{<w>}}(23 + x)/2 = 27\textcolor{red}{\texttt{<w>}}To find x, I should solve this equation. Let me multiply both sides by 2 to get rid of the denominator. That gives:\textcolor{red}{\texttt{<w>}}23 + x = 54\textcolor{red}{\texttt{<w>}}Then, subtract 23 from both sides to isolate x:\textcolor{red}{\texttt{<w>}}x = 54 - 23\textcolor{red}{\texttt{<w>}}Calculating that, 54 minus 23 is 31. So x is 31. Now, the question asks for the positive difference between 23 and x. The positive difference would be the absolute value of 23 - x. Since x is 31, that's |23 - 31|, which is | -8 |, so 8. Alternatively, it could also be |31 - 23|, which is the same result, 8. Either way, the positive difference is 8.\textcolor{red}{\texttt{<w>}}Wait, let me check my steps again to make sure I didn't make a mistake. Starting with the average: (23 + x)/2 = 27. Multiply both sides by 2: 23 + x = 54. Subtract 23: x = 31. Difference between 23 and 31 is 8. That seems right. Yeah, I think that's correct. No issues here.\textcolor{red}{\texttt{<w>}}
\texttt{<|end\_of\_thought|>}

\texttt{<|begin\_of\_solution|>}
\textcolor{red}{\texttt{<w>}}The average of 23 and \( x \) is given by \(\frac{23 + x}{2} = 27\). Multiplying both sides by 2:  
\[
23 + x = 54
\]  
Subtracting 23 from both sides:  
\[
x = 54 - 23 = 31
\]  
The positive difference between 23 and \( x \) is:  
\[
|31 - 23| = 8
\]  \textcolor{red}{\texttt{<w>}}\(\boxed{8}\)
\texttt{<|end\_of\_solution|>}

\end{tcolorbox}
}

\caption{A training case. \texttt{<w>} is a compression trigger.}
\label{prompt:case:train}
\end{figure*}

==> tables/app_comparision.tex <==
\begin{table*}[h!]
\small
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{Method} & \textbf{Memory Optimization} & \textbf{Training Cost} & \textbf{Interpretability} & \textbf{Generalization} \\
\midrule
System-1.5~\cite{arxiv25_system_1_5} & Significant & High  & Weak & Weak \\
SoftThinking~\cite{arxiv25_soft_thinking}  & Limited    & None  & Weak & Good \\
\ours & Significant & Low   & Good & Good \\
\bottomrule
\end{tabular}
\caption{Comparison of different methods.}
\label{tab:app:comparison}
\end{table*}


==> tables/exp_compression_count.tex <==
\begin{table}[]
\centering
\small
\scalebox{1}{
\begin{tabular}{ccccc}
\toprule
      & GSM8K & MMLU & GPQA & BBH \\ \midrule
Qwen  & 20    & 37   & 115  & 48  \\
Llama & 26    & 47   & 139  & 55  \\ \bottomrule
\end{tabular}
}
\caption{
Statistics of the average number of compressions per dataset for \ours.
}
\label{table:exp:efficiency:comp_count}
\vspace{-2mm}
\end{table}

==> tables/exp_same_memory.tex <==
\begin{table}[]
\centering
\small
\scalebox{0.85}{
\begin{tabular}{cccccc}
\toprule
             & GSM8K & MMLU  & GPQA  & BBH   & AVG   \\ \midrule
Vanilla      & 11.83 & 20.61 & 10.76 & 11.50 & 13.68 \\
LightThinker & \textbf{6.73}  & \textbf{7.44}  & \textbf{3.86}  & \textbf{3.97}  & \textbf{5.50}  \\ \bottomrule
\end{tabular}
}
\caption{
 Inference time comparison (in hours) for Vanilla and \ours~on the Qwen model across four datasets under the same memory budget.
}
\vspace{-0.5cm}
\label{table:exp:efficiency:same_memory}
\end{table}
